HSDF-Lane: Height-Aligned Signed Distance Field with Semantic Lane Prior for 3D Lane Detection

Monocular 3D lane detection plays a critical role in autonomous driving, yet recovering reliable 3D geometry from a single image remains challenging due to inherent depth ambiguity. Prior methods project image features into Bird's-Eye-View (BEV) space under a flat-ground assumption, causing geometric distortion on real-world roads. Recent methods instead predict explicit height maps to capture non-planar surfaces, but still rely on sparse anchor-based regression and exploit the recovered geometry merely for spatial transformation rather than semantic understanding. To overcome these limitations, we propose HSDF-Lane, which implicitly models the road surface as a Height-aligned Signed Distance Field (HSDF) over a densely sampled 3D feature volume. Through differentiable rendering, the HSDF jointly produces an accurate height map and surface-aligned features. We further introduce Lane-aware Semantic Positional Encoding (LSPE), which injects a lane-existence prior derived from the surface-aligned features into the transformer queries, coupling geometric structure with semantic guidance. Extensive experiments on the OpenLane benchmark show that HSDF-Lane achieves state-of-the-art performance in both 3D lane detection and height map estimation.

==> Misc/header.tex <==
\newcommand{\jbi}[1]{\textcolor{red}{(jbi: #1)}}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{{vs}\onedot}
\def\wrt{\emph{w.r.t}\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\def\aka{\emph{a.k.a}\onedot}

% https://www.overleaf.com/project/5c3ee6aa83e7382dd5ccc228
\newcommand{\Tref}[1]{Table~\textcolor{eccvblue}{\ref{#1}}}
\newcommand{\Eref}[1]{Eq.~\textcolor{eccvblue}{\ref{#1}}}
\newcommand{\Fref}[1]{Fig.~\textcolor{eccvblue}{\ref{#1}}}
\newcommand{\Sref}[1]{Sec.~\textcolor{eccvblue}{\ref{#1}}}
\newcommand{\Aref}[1]{Alg.~\textcolor{eccvblue}{\ref{#1}}}

% this is changed due to the default option of 3DV format
\usepackage[dvipsnames]{xcolor}
%\usepackage{xcolor}
\definecolor{grey}{rgb}{0.52,0.52,0.52}

\usepackage{comment}

% Beautiful table
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{verbatim}
\usepackage{hhline}
\usepackage{multirow}
\usepackage{makecell}

% for rebuttal
\definecolor{R1}{rgb}{0.0, 0.5, 1.0}
\definecolor{R2}{HTML}{00893d}
\definecolor{R3}{RGB}{120, 20, 180} %violet-ish
\newcommand{\responseOne}[2]{\vspace{4pt}\noindent\textbf{[\textcolor{#1}{#1}]~#2:}}
\newcommand{\responseTwo}[3]{\vspace{4pt}\noindent\textbf{[\textcolor{#1}{#1},\textcolor{#2}{#2}]~#3:}}
\newcommand{\responseAll}[1]{\vspace{4pt}\noindent\textbf{[\textcolor{R1}{R1},\textcolor{R2}{R2},\textcolor{R3}{R3}]~#1:}}

